Improved Estimation of Ranks for Learning Item Recommenders with Negative Sampling

In recommendation systems, there has been a growth in the number of recommendable items (# of movies, music, products). When the set of recommendable items is large, training and evaluation of item recommendation models becomes computationally expensive. To lower this cost, it has become common to sample negative items. However, the recommendation quality can suffer from biases introduced by traditional negative sampling mechanisms. In this work, we demonstrate the benefits from correcting the bias introduced by sampling of negatives. We first provide sampled batch version of the well-studied WARP and LambdaRank methods. Then, we present how these methods can benefit from improved ranking estimates. Finally, we evaluate the recommendation quality as a result of correcting rank estimates and demonstrate that WARP and LambdaRank can be learned efficiently with negative sampling and our proposed correction technique.

==> method.tex <==

\subsection{WARP and \lambdarank}

\begin{algorithm}[t]
  \caption{Iterative Pairwise Training}\label{algo:iterative}
  \begin{algorithmic}[1]
  \State \textbf{Input:} dataset $\setS$, learning rate $\eta$
  \State \textbf{Output:} model parameters $\theta$
%  \BlankLine
  \Repeat
    \State sample $(c,i) \sim \setS$ \Comment{positive observation}
    \State sample $j \sim \setI$ with probability $q(j|c,i)$ \Comment{negative item} \label{line:draw_neg}
    \State $\theta \leftarrow \theta - \eta \, \alpha(c,i,j)\frac{\partial}{\partial \theta}l(c,i,j)$ \Comment{gradient step}
  \Until{Convergence}
  \State \textbf{return} $\theta$
  \end{algorithmic}
\end{algorithm}


WARP and \lambdarank are iterative algorithms that draw one positive observation and one negative observation and apply a gradient step on this sampled pair of items.
See algorithm~\ref{algo:iterative} for a generalized algorithm~\cite{rendle:implicit}.
WARP and \lambdarank differ in (i)~how they sample the negative item (i.e., in $q$) and (ii)~how they weight the update (i.e., $\alpha$). 
We will discuss these two choices next.
For WARP, the negative item is drawn with a rejection sampling algorithm.
In particular, WARP draws candidate items uniformly until it finds a candidate $j$ such that $l(c,i,j) > 0$, where $l$ is a pairwise loss function (see eqs.~\ref{eq:hinge} and \ref{eq:logistic})
If the rejection algorithm cannot find a candidate in predefined number of steps, it will exit and discard the step.
For \lambdarank, negative items are drawn uniformly without any rejection step, i.e., $q(j|c,i) = \frac{1}{|\setI|-1}$.

The weighting function, $\alpha$ of \lambdarank depends on the rank $\rank(i)$ of the positive item $i$ and the rank of the negative item $j$ and $\alpha(c,i,j)=\ndcg(j)-\ndcg(i)$.
This rank is computed over all items $\setI$.
The weighting function, $\alpha$ of WARP depends only on the rank of the positive item $i$.
However instead of computing this rank over all items, WARP uses estimates this rank based on how many steps the rejection algorithm was run.
The estimated rank is $...$.
The weighting function is $\alpha(c,i,j)= \sum_{r=1}^{\rank(i)} \frac{1}{r}$.

WARP employs usually a pairwise hinge loss, i.e.,
\begin{align}
    l(c,i,j) = \max(0, \hy(c,i) - \hy(c,j)) \label{eq:hinge}
\end{align}
and \lambdarank a pairwise logistic loss
\begin{align}
    l(c,i,j) = \ln\sigma(\hy(c,i) - \hy(c,j)). \label{eq:logistic}
\end{align}
We want to highlight that computing the rank is a crucial operation for \lambdarank and WARP.
For \lambdarank this is computationally expensive because it computes the rank over all items.
This becomes costly for large catalogs.
WARP computes the rank through the rejection sampling algorithm.
Again, if the item is ranked high and the item catalog is large, this operation is costly.



\section{Batch Training with Negative Sampling}

\begin{algorithm}[t]
  \caption{Sampled Batch Training}\label{algo:batch}
  \begin{algorithmic}[1]
  \State \textbf{Input:} dataset $\setS$, learning rate $\eta$
  \State \textbf{Output:} model parameters $\theta$
%  \BlankLine
  \Repeat
    \State sample $\tilde{\setS} \sim 2^\setS $ s.th. $ |\tilde{\setS}|=k$ \Comment{positive observations}
    \State sample $\tilde{\setI} \sim 2^\setI $ s.th. $ |\tilde{\setI}|=m$ \Comment{negative items}
    \State $\theta \leftarrow \theta - \eta \, \sum_{j \in \tilde{\setI}}\sum_{(c,i) \in \tilde{\setS}}\alpha(c,i,j)\frac{\partial}{\partial \theta}l(c,i,j)$ \Comment{grad. step}
  \Until{Convergence}
  \State \textbf{return} $\theta$
  \end{algorithmic}
\end{algorithm}


Modern training algorithms make use of hardware that is designed for parallel execution.
The WARP and LambdaRank algorithms discussed so far are not well suited for modern hardware as they process one item at a time.
Especially the iterative rejection sampling algorithm of WARP is not a good fit.
We will propose now a simple variant that process several negative and positive items in parallel.
Algorithm~\ref{algo:batch} shows the generalized algorithm.
It simply samples uniformly batches of $k$ positives and $m$ negatives.
A gradient step is applied to all $k \times m$ pairs.
This operation is better suited for parallel execution.

We note that the sampled batch training algorithm samples uniformly and does not reject any negative items like the iterative WARP algorithm.
However, even in the original iterative WARP algorithm, the gradient steps would not change if the rejection algorithm would accept all items because accepting an item with $l(c,i,j)=0$ would anyway have a gradient of 0 for the hinge loss.
So the purpose of the rejection algorithm in WARP is mostly to compute the rank.
For sampled batch training, we can use other ways to estimate ranks and can therefore remove the rejection algorithm.



\subsection{Estimation of Rank}



To better deal with large item catalogs, we rank items within the sampled set $\tilde\setI$ of negative items instead of computing the rank on the full catalog which would be very costly.
%Estimating the rank from the subset of negative samples introduces a bias.
We define the rank in the sample $\tilde\setI$ as
\begin{align}
    \tilde{\rank}_{\tilde\setI}(i |c) =  |\{ j \in \tilde{\setI}: \hy(c,j) > \hy(c,i) \}|  \label{eq:rank_subsample}
\end{align}
and refer to it as the \emph{sampled rank}.
The sampled rank from a subset $\tilde\setI \subset \setI$ is a poor estimate of the true rank, $\rank$.
For example, the maximum rank is $m$ instead of $|\setI|$.
In general, it underestimates the rank because some of the items that are ranked above $i$ might be missing from $\tilde\setI$. % TODO: this assumes sampling without replacement

We will follow the ideas from \cite{krichene:sampled_metrics} that have previously analyzed this issue and provided correction methods in the context of evaluating with sampled metrics.
%We will outline this next.
The sampled rank, $\tilde{\rank}$ is a random variable that depends on the sampled set of negatives.
The sampled rank counts how often a sampled item is ranked above the positive item.
If negative items are sampled uniformly, then the probability of sampling a negative item ranking above the positive item depends on the true rank of the positive item and the probability is:
\begin{align}
    p(\rank(j|c) > \rank(i|c)) = \frac{\rank(i|c) -1}{|\setI| - 1} 
\end{align}
The rank on the subsample (eq.~\ref{eq:rank_subsample}) repeats this process $m$ times and counts the successes.
Thus the rank on the subsample is binomial distributed:
\begin{align}
    \tilde{\rank}(i | c) \sim B\left(m, p\right) + 1, \quad p = \frac{\rank(i|c) - 1}{|\setI| - 1}
\end{align}
The probability $p$ can be estimated from the sampled rank by:
\begin{align}
    \hat{p} = \frac{ \tilde{\rank}(i | c) -1}{m}
\end{align}
And thus, an estimator of the rank on the full catalog is
\begin{align}
    \hat{\rank}(i|c) = 1 + \frac{ \tilde{\rank}(i | c) -1}{m} (n-1) .
\end{align}
The estimated rank $\hat{\rank}$ is a better estimator of the true rank $\rank$ than the sampled rank $\tilde\rank$.
In Section~\ref{sec:experiments}, we compare batch training of WARP and \lambdarank with the sampled rank and the estimated rank.

\subsection{Discussion}
An alternative to estimating the rank, $\hat{\rank}$, would be to estimate $\hat{\alpha}$ from the sampled ranks.
This could follow the ideas of \cite{krichene:sampled_metrics} for estimating a corrected metric from sampled ranks.
For example, for \lambdarank, $\alpha$ is a function of the $\ndcg$ and \cite{krichene:sampled_metrics} suggested method for estimating the $\ndcg$ metric from sampled ranks $\tilde{\rank}$.
This is a promising direction for future work.

